Catalog of Energy Patterns for Mobile Applications

Software engineers make use of design patterns for reasons that range from performance to code comprehensibility. Several design patterns capturing the body of knowledge of best practices have been proposed in the past, namely creational, structural and behavioral patterns. However, with the advent of mobile devices, it becomes a necessity a catalog of design patterns for energy efficiency. In this work, we inspect commits, issues and pull requests of 1027 Android and 756 iOS apps to identify common practices when improving energy efficiency. This analysis yielded a catalog, available online, with 22 design patterns related to improving the energy efficiency of mobile apps. We argue that this catalog might be of relevance to other domains such as Cyber-Physical Systems and Internet of Things. As a side contribution, an analysis of the differences between Android and iOS devices shows that the Android community is more energy-aware.

==> reports/app_stars.tex <==
\begin{tabular}{llrrrrrrr}
\hline
                   & Platform   &    Mean &      Std &   Min &   25\% &   Median &    75\% &        Max \\
\hline
 Stars             & Android    &   145.3 &    608.6 &   0.0 &   6.0 &     20.0 &   68.0 &    15159.0 \\
 Stars             & iOS        &   486.8 &   1272.5 &   0.0 &  18.2 &     71.0 &  329.8 &    15318.0 \\
 Forks             & Android    &    75.4 &    302.2 &   0.0 &   4.0 &     14.0 &   46.8 &     7811.0 \\
 Forks             & iOS        &   118.1 &    354.0 &   0.0 &   7.0 &     20.0 &   71.0 &     4820.0 \\
 Number of Reviews & Android    & 31855.2 & 529676.3 &   1.0 &  24.0 &    138.0 & 1087.0 & 13080790.0 \\
 Number of Reviews & iOS        &  3241.8 &  12597.0 &   5.0 &  18.0 &     75.0 & 1038.5 &   115011.0 \\
 Rating            & Android    &     3.8 &      0.5 &   1.0 &   4.0 &      4.0 &    4.0 &        5.0 \\
 Rating            & iOS        &     4.1 &      0.7 &   2.0 &   3.6 &      4.0 &    4.5 &        5.0 \\
\hline
\end{tabular}
